Oscillation properties of one boundary problem of fourth order with a spectral parameter in the boundary conditions

For one boundary problem of fourth order with a spectral parameter in the boundary condition we prove the simplicity of the spectrum and the oscillation properties of the system of the eigenfunctions derivatives.

==> vladimi.tex <==
\input plainenc
\input amssym
\fontencoding{T2A}
\inputencoding{utf-8}
\tolerance 4000
\binoppenalty 10000
\relpenalty 10000
\parindent 1.5em

\catcode`\@ 11
\font\TITLE labx1440
\font\tenrm larm1000
\font\cmtenrm cmr10
\font\tenit lati1000
\font\tenbf labx1000
\font\tentt latt1000
\font\teni cmmi10 \skewchar\teni '177
\font\tensy cmsy10 \skewchar\tensy '60
\font\tenex cmex10
\font\teneufm eufm10
\font\tenmsb msbm10
\font\ninerm larm0900
\font\cmninerm cmr9
\font\nineit lati0900
\font\ninebf labx0900
\font\ninei cmmi9 \skewchar\ninei '177
\font\ninesy cmsy9 \skewchar\ninesy '60
\font\nineex cmex9
\font\nineeufm eufm9
\font\ninemsb msbm9
\font\eightrm larm0800
\font\cmeightrm cmr8
\font\eightit lati0800
\font\eightbf labx0800
\font\eighti cmmi8 \skewchar\eighti '177
\font\eightsy cmsy8 \skewchar\eightsy '60
\font\eightex cmex8
\font\eighteufm eufm8
\font\eightmsb msbm8
\font\sevenrm larm0700
\font\cmsevenrm cmr7
\font\sevenit lati0700
\font\sevenbf labx0700
\font\seventt latt0700
\font\seveni cmmi7 \skewchar\seveni '177
\font\sevensy cmsy7 \skewchar\sevensy '60
\font\sevenex cmex7
\font\seveneufm eufm7
\font\sevenmsb msbm7
\font\cmsixrm cmr6
\font\sixbf labx0600
\font\sixi cmmi6 \skewchar\sixi '177
\font\sixsy cmsy6 \skewchar\sixsy '60
\font\sixeufm eufm6
\font\sixmsb msbm6
\font\cmfiverm cmr5
\font\fivebf labx0500
\font\fivei cmmi5 \skewchar\fivei '177
\font\fivesy cmsy5 \skewchar\fivesy '60
\font\fiveeufm eufm5
\font\fivemsb msbm5
\font\tencmmib cmmib10 \skewchar\tencmmib '177
\font\ninecmmib cmmib9 \skewchar\ninecmmib '177
\font\eightcmmib cmmib8 \skewchar\eightcmmib '177
\font\sevencmmib cmmib7 \skewchar\sevencmmib '177
\font\sixcmmib cmmib6 \skewchar\sixcmmib '177
\font\fivecmmib cmmib5 \skewchar\fivecmmib '177
\newfam\cmmibfam
\textfont\cmmibfam\tencmmib \scriptfont\cmmibfam\sevencmmib
\scriptscriptfont\cmmibfam\fivecmmib
\def\tenpoint{\def\rm{\fam0\tenrm}\def\it{\fam\itfam\tenit}%
	\def\bf{\fam\bffam\tenbf}\def\tt{\fam\ttfam\tentt}%
	\textfont0\cmtenrm \scriptfont0\cmsevenrm \scriptscriptfont0\cmfiverm%
	\textfont1\teni \scriptfont1\seveni \scriptscriptfont1\fivei%
	\textfont2\tensy \scriptfont2\sevensy \scriptscriptfont2\fivesy%
	\textfont3\tenex \scriptfont3\tenex \scriptscriptfont3\tenex%
	\textfont\itfam\tenit%
	\textfont\bffam\tenbf \scriptfont\bffam\sevenbf%
	\scriptscriptfont\bffam\fivebf%
	\textfont\eufmfam\teneufm \scriptfont\eufmfam\seveneufm%
	\scriptscriptfont\eufmfam\fiveeufm%
	\textfont\msbfam\tenmsb\scriptfont\msbfam\sevenmsb%
	\scriptscriptfont\msbfam\fivemsb%
	\textfont\cmmibfam\tencmmib \scriptfont\cmmibfam\sevencmmib%
	\scriptscriptfont\cmmibfam\fivecmmib%
	\normalbaselineskip 12pt%
	\setbox\strutbox\hbox{\vrule height8.5pt depth3.5pt width0pt}%
	\normalbaselines\rm}
\def\ninepoint{\def\rm{\fam 0\ninerm}\def\it{\fam\itfam\nineit}%
	\def\bf{\fam\bffam\ninebf}%
	\textfont0\cmninerm \scriptfont0\cmsixrm
	\textfont1\ninei \scriptfont1\sixi
	\textfont2\ninesy \scriptfont2\sixsy
	\textfont3\nineex \scriptfont3\nineex \scriptscriptfont3\nineex
	\textfont\itfam\nineit
	\textfont\bffam\ninebf \scriptfont\bffam\sixbf
	\textfont\eufmfam\nineeufm \scriptfont\eufmfam\sixeufm
	\textfont\msbfam\ninemsb\scriptfont\msbfam\sixmsb%
	\scriptscriptfont\msbfam\fivemsb%
	\textfont\cmmibfam\ninecmmib \scriptfont\cmmibfam\sixcmmib}
\def\eightpoint{\def\rm{\fam 0\eightrm}\def\it{\fam\itfam\eightit}%
	\def\bf{\fam\bffam\eightbf}%
	\textfont0\cmeightrm \scriptfont0\cmfiverm \scriptscriptfont0\cmfiverm%
	\textfont1\eighti \scriptfont1\fivei \scriptscriptfont1\fivei%
	\textfont2\eightsy \scriptfont2\fivesy \scriptscriptfont2\fivesy%
	\textfont3\eightex \scriptfont3\eightex \scriptscriptfont3\eightex%
	\textfont\itfam\eightit%
	\textfont\bffam\eightbf \scriptfont\bffam\fivebf%
	\scriptscriptfont\bffam\fivebf%
	\textfont\eufmfam\eighteufm \scriptfont\eufmfam\fiveeufm%
	\scriptscriptfont\eufmfam\fiveeufm%
	\textfont\msbfam\eightmsb\scriptfont\msbfam\fivemsb%
	\scriptscriptfont\msbfam\fivemsb%
	\textfont\cmmibfam\eightcmmib \scriptfont\cmmibfam\fivecmmib%
	\scriptscriptfont\cmmibfam\fivecmmib%
	\normalbaselineskip 11pt%
	\abovedisplayskip 5pt%
	\belowdisplayskip 5pt%
	\setbox\strutbox\hbox{\vrule height7pt depth2pt width0pt}%
	\normalbaselines\rm}

\def\No{\char 157}
\def\empty{}

\catcode`\" 12
\def\k@vy{"}
\def\bolddelta{\mathchar"0\hexnumber@\cmmibfam 0E}
\def\acute{\mathaccent"7013 }
\def\grave{\mathaccent"7012 }
\def\ddot{\mathaccent"707F }
\def\tilde{\mathaccent"707E }
\def\bar{\mathaccent"7016 }
\def\breve{\mathaccent"7015 }
\def\check{\mathaccent"7014 }
\def\hat{\mathaccent"705E }
\def\vec{\mathaccent"017E }
\def\dot{\mathaccent"705F }
\def\widetilde{\mathaccent"0365 }
\def\widehat{\mathaccent"0362 }
\catcode`\" 13
\def"#1{\ifx#1<\char 190\relax\else\ifx#1>\char 191\relax\else%
	\ifx#1`\char 16\relax\else\ifx#1'\char 17\relax\else #1\fi\fi\fi\fi}

\long\def\hyp@rprov#1#2#3#4{\hbox{\ifx\hyperrefs\undefined #1\else%
	\special{html:<a #2>}\ifx#3\relax\else\special{color push #4}\fi #1%
	\ifx#3\relax\else\special{color pop}\fi\special{html:</a>}\fi}}

\newcount\c@section
\newcount\c@subsection
\newcount\c@subsubsection
\newcount\c@equation
\newcount\c@bibl
\newcount\c@enum
\c@section 0
\c@subsection 0
\c@subsubsection 0
\c@equation 0
\c@bibl 0
\newdimen\d@enum
\d@enum 0pt
\def\lab@l{}
\def\label#1{\immediate\write 11{\string\newl@bel{#1}{\lab@l}}\ifhmode\unskip\fi}
\def\eqlabel#1{\rlap{$(\equation)$}\label{#1}}
\def\bibitem#1{\global\advance\c@bibl 1\par\noindent{\hyp@rprov{%
	\ninerm [\number\c@bibl]}{name=\k@vy cite:\number\c@bibl\k@vy}\relax{}~}%
	\immediate\write 11{\string\newbl@bel{#1}{\number\c@bibl}}}

\def\section#1{\global\advance\c@section 1
	{\par\vskip 3ex plus 0.5ex minus 0.1ex
	\rightskip 0pt plus 1fill\leftskip 0pt plus 1fill\noindent
	\hyp@rprov{{\bf\S\thinspace\number\c@section .~#1}}{%
	name=\k@vy sect:\number\c@section\k@vy}%
	\relax{}\par\penalty 10000\vskip 1ex plus 0.25ex}
	\gdef\lab@l{\number\c@section.:\number\pageno}
	\c@subsection 0
	\c@subsubsection 0
	\c@equation 0
}
\def\subsection{\global\advance\c@subsection 1
	\par\vskip 1ex plus 0.1ex minus 0.05ex\indent
	\hyp@rprov{{\bf\number\c@subsection.{}}}{%
	name=\k@vy sect:\number\c@section.\number\c@subsection\k@vy}\relax{}%
	\gdef\lab@l{\number\c@section.\number\c@subsection:\number\pageno}
	\c@subsubsection 0
}
\def\subsubsection{\global\advance\c@subsubsection 1
	\par\vskip 1ex plus 0.1ex minus 0.05ex\indent%
	\hyp@rprov{{\bf\number\c@subsection.\number\c@subsubsection.{}}}{%
	name=\k@vy sect:\number\c@section.\number\c@subsection.%
	\number\c@subsubsection\k@vy}\relax{}%
	\gdef\lab@l{\number\c@section.\number\c@subsection.%
		\number\c@subsubsection:\number\pageno}
}
\def\equation{\global\advance\c@equation 1
	\gdef\lab@l{\number\c@section.\number\c@equation:\number\pageno}
	\hyp@rprov{{\rm\number\c@equation}}{name=\k@vy eq:\number\c@section(%
	\number\c@equation)\k@vy}\relax{}%
}
\catcode`\# 11
\def\sh@rp{#}
\catcode`\# 6
\def\ref@ref#1.#2:#3:{\def\REF@{#2}\ifx\REF@\empty%
	\hyp@rprov{{\rm \S\thinspace#1}}{href=\k@vy\sh@rp sect:#1\k@vy}0{rgb 0 0 1}%
	\else\hyp@rprov{\ifnum #1=\c@section {\rm #2}%
	\else {\rm \S\thinspace#1.#2}\fi}{href=\k@vy\sh@rp sect:#1.#2\k@vy}0{rgb 0 0 1}\fi
}
\def\ref@pageref#1:#2:{#2}
\def\ref@eqref#1.#2:#3:{\hyp@rprov{\ifnum #1=\c@section {\rm (#2)}\else%
	{\rm \S\thinspace#1$\,$(#2)}\fi}{href=\k@vy\sh@rp eq:#1(#2)\k@vy}0{rgb 0 0 1}%
}
\def\ref#1{\expandafter\ifx\csname l@#1\endcsname\relax
	{\bf ??}\message{^^J Reference #1 undefined!^^J}%
	\else\edef\mur@{\csname l@#1\endcsname :}%
	{\expandafter\ref@ref\mur@}\fi}
\def\pageref#1{\expandafter\ifx\csname l@#1\endcsname\relax
	{\bf ??}\message{^^J Reference #1 undefined!^^J}%
	\else\edef\mur@{\csname l@#1\endcsname :}%
	{\expandafter\ref@pageref\mur@}\fi}
\def\eqref#1{\expandafter\ifx\csname l@#1\endcsname\relax
	{(\bf ??)}\message{^^J Reference (#1) undefined!^^J}%
	\else\edef\mur@{\csname l@#1\endcsname :}%
	{\expandafter\ref@eqref\mur@}\fi}
\def\cite#1{\expandafter\ifx\csname bl@#1\endcsname\relax
	{\bf ??}\message{^^J Citation #1 undefined!^^J}%
	\else\hyp@rprov{{\bf\csname bl@#1\endcsname}}{href=\k@vy\sh@rp cite:%
	\expandafter\number\csname bl@#1\endcsname\k@vy}0{rgb 0 0 1}\fi}

\def\dfrac#1#2{{\displaystyle #1\over\displaystyle #2}}
\def\superalign#1{\openup 1\jot\tabskip 0pt\halign to\displaywidth{%
	\tabskip 0pt plus 1fil$\displaystyle ##$&%
	\tabskip 0pt\hss $\displaystyle ##{}$&%
	$\displaystyle {}##$\hss\tabskip 0pt plus 1fil&%
	\tabskip 0pt\hss ##\crcr #1\crcr}}
\long\def\enumerate#1#2{%
	\setbox0\hbox{$#1^{\circ}.\ $}\d@enum\wd0\global\advance\d@enum 2pt\c@enum 0%
	{\def\item{\global\advance\c@enum 1\par\hskip 0pt%
	\hbox to \d@enum{$\number\c@enum^{\circ}$.\hss}}%
	\par\smallskip #2\par\smallskip}
}
\def\Wo{{\mathpalette\Wo@{}}W}
\def\Wo@#1{\setbox0\hbox{$#1 W$}\dimen@\ht0\dimen@ii\wd0\raise0.65\dimen@%
\rlap{\kern0.35\dimen@ii$#1{}^\circ$}}
\catcode`\@ 12

\def\proof{\par\medskip{\rm Д$\,$о$\,$к$\,$а$\,$з$\,$а$\,$т$\,$е$\,$%
	л$\,$ь$\,$с$\,$т$\,$в$\,$о.}\ }
\def\endproof{{\parfillskip 0pt\hfill$\square$\par}\medskip}

\def\newl@bel#1#2{\expandafter\gdef\csname l@#1\endcsname{#2}}
\def\newbl@bel#1#2{\expandafter\gdef\csname bl@#1\endcsname{#2}}
\def\contentsline#1#2#3{\expandafter\gdef\csname contents@\number\c@content%
	\endcsname{\par\ifnum #1=0\vskip 4pt\else\vskip 1pt\fi\noindent%
	\hbox to \hsize{\ifnum #1=0{\bf #2\thinspace}\else\hskip 0.5cm%
	#2\thinspace\fi\leaders\hbox to 0.25cm{.}\hfill #3}}%
	\global\advance\c@content 1
}
\openin 11=\jobname .aux
\ifeof 11
	\closein 11\relax
\else
	\closein 11
	\input\jobname .aux
	\relax
\fi

\immediate\openout 11=\jobname.aux

